Extremal storage functions and minimal realizations of discrete-time linear switching systems

We study the $\mathcal{L}_p$ induced gain of discrete-time linear switching systems with graph-constrained switching sequences. We first prove that, for stable systems in a minimal realization, for every $p \geq 1$, the $\mathcal{L}_p$-gain is exactly characterized through switching storage functions. These functions are shown to be the $p$th power of a norm. In order to consider general systems, we provide an algorithm for computing minimal realizations. These realizations are \emph{rectangular systems}, with a state dimension that varies according to the mode of the system. We apply our tools to the study on the of $\mathcal{L}_2$-gain. We provide algorithms for its approximation, and provide a converse result for the existence of quadratic switching storage functions. We finally illustrate the results with a physically motivated example.

==> header.tex <==
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}							% Input encoding
\usepackage{amsmath}									% Math
\usepackage{amssymb}
\usepackage[usenames,dvipsnames]{color}
\usepackage{multicol}
\usepackage[lined,boxed]{algorithm2e}
\usepackage[hidelinks]{hyperref}
\usepackage{graphicx}	
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{caption}
\usepackage{subcaption}

\usepackage[outdir = ./]{epstopdf} 
	\DeclareGraphicsExtensions{.pdf,.png,.jpg,.eps}

\usepackage{cite}
\usepackage{xcolor}


